On fractal patterns in Ulam words

Ulam words are binary words defined recursively as follows: the length-$1$ Ulam words are $0$ and $1$, and a binary word of length $n$ is Ulam if and only if it is expressible uniquely as a concatenation of two shorter, distinct Ulam words. We discover, fully describe, and prove a surprisingly rich structure already in the set of Ulam words containing exactly two $1$'s. In particular, this leads to a complete description of such words and a logarithmic-time algorithm to determine whether a binary word with two $1$'s is Ulam. Along the way, we uncover delicate parity and biperiodicity properties, as well as sharp bounds on the number of $0$'s outside the two $1$'s. We also show that sets of Ulam words indexed by the number $y$ of $0$'s between the two $1$'s have intricate tensor-based hierarchical structures determined by the arithmetic properties of $y$. This allows us to construct an infinite family of self-similar Ulam-word-based fractals indexed by the set of $2$-adic integers, containing the outward Sierpinski gasket as a special case.

==> conclusion.tex <==
\section{Conclusion}


==> conjecture.tex <==
\section{An interesting conjecture}\label{conjecture}
For many sequences, one of their most revealing properties is their density. Some have positive asymptotic density; others have $0.$ Even with those sequences with zero density, it is interesting to examine, asymptotically, how exactly they behave. 

Ulam words possess the unwieldy property that their counts become exponentially large---there are more than $200,000$ Ulam words of length $20$ \cite[A337361]{oeis}. Therefore, it is unfeasible to exactly calculate (the size of) $\UU(n)$ for $n$ larger than, say, $30.$ However, a probabilistic algorithm run with many trials allows us to approximate its density. Precisely, we can randomly sample binary sequences of length $n$ and count the number of instances in which those sequences are Ulam. Determining whether a word of length $n$ is Ulam, however, takes $O(n^3)$ time, since we have to test all possible sub-words for Ulamness, and each sub-word can be separated into two in $O(n)$ ways. Afterwards, there exist a variety of tests calculating the expected probability that a random word of length $n$ is Ulam. 
\begin{table}[H]
    \centering
    \begin{tabular}{rr||c|c|c}
         && Number of Trials & Number Ulam & Proportion (90\% confidence) \\
         \hline
         &&\\[-2ex]
         & 20 & 1048576 & 225166 & $0.2147$ (exact) \\
         & 25 & 33554432 & 6720784 & $0.2003$ (exact) \\
         & 50 & 100000000 & 15942011 & $0.15942\pm0.00006$ \\
         & 75 & 50000000 & 6790245 & $0.1358\pm0.00008$ \\
         \raisebox{\dimexpr0pt}[0pt][0pt]
         {\rotatebox[origin=c]
         {90}
         {Length of word}} & 100 & 20000000 & 2406053 & $0.1203\pm0.0001$ \\
         & 150 & 10000000 & 1008389 & $0.10084\pm0.00016$ \\
         & 200 & 6000000 & 530582 & $0.0885\pm0.0003$ \\
         & 300 & 500000 & 36521 & $0.0730\pm0.0006$ \\
         & 500 & 100000 & 5855 & $0.05855\pm0.0012$ \\
         & 1000 & 90000 & 3650 & $0.0406\pm0.0013$
    \end{tabular}
    \caption{%\centering 
    Experimentally calculated proportions of Ulam words of length $n$\\Calculated using Wilson's test \cite{wilson-test}}
    \label{tab:my_label}
\end{table}
The proportions in the table become asymptotically close to $\left(\frac{3}{4}\right)^{\log_2(n)+1}=\frac{0.75}{n^{\log_2(4/3)}}.$ 

Evidence for this precise proportionality is given by calculating proportions of Ulam words containing exactly one or exactly two $1$'s. Recall that the $k$-th element of the $n$-th row is included if and only if $k$ has $0$'s in all places where $n$ does in its binary representation. In particular, if $n$ is made to range up to $2^d,$ then there are $d$ spots in the binary representations for $n$ and $k.$ For each spot, it is either $0$ in both $n$ and $k,$ or $0$ in $k$ but not $n,$ or $1$ in both $n$ and $k.$ Thus, there are three choices for it and so in total there are $3^d$ choices for $n$ and $k$ such that $w(n,k)$ is Ulam. In particular, we see that, for any number $n$ between $2^d$ and $2^{d+1},$ the number of Ulam words of length up to $n$ is bounded below by $3^d$ and above by $3^{d+1}.$ In any case, the proportion of Ulam words is then $\Theta\left(\frac{3^{\log_2n}}{n^2}\right)=\Theta\left(\frac{1}{n^{\log_2(4/3)}}\right).$ To understand the same proportionality for Ulam words with two $1$'s, we have to work slightly harder.

\begin{lemma}

\end{lemma}

==> side-thm.tex <==
\section{Additional Results}\label{side-thm}
\begin{prop}
The word $0^x1^y$ is Ulam if and only if either $x+y=1$ or $x,y\geq1$ and $\binom{x+y-2}{x-1}$ is odd.
\end{prop}
\begin{proof}

\end{proof}
